Composition constraints of the TRAPPIST-1 planets from their formation

We study the formation of the TRAPPIST-1 (T1) planets starting shortly after Moon-sized bodies form just exterior to the ice line. Our model includes mass growth from pebble accretion and mergers, fragmentation, type-I migration, and eccentricity and inclination dampening from gas drag. We follow the composition evolution of the planets fed by a dust condensation code that tracks how various dust species condense out of the disc as it cools. We use the final planet compositions to calculate the resulting radii of the planets using a new planet interior structure code and explore various interior structure models. Our model reproduces the broader architecture of the T1 system and constrains the initial water mass fraction of the early embryos and the final relative abundances of the major refractory elements. We find that the inner two planets likely experienced giant impacts and fragments from collisions between planetary embryos often seed the small planets that subsequently grow through pebble accretion. Using our composition constraints we find solutions for a two-layer model, a planet comprised of only a core and mantle, that match observed bulk densities for the two inner planets b and c. This, along with the high number of giant impacts the inner planets experienced, is consistent with recent observations that these planets are likely dessicated. However, two-layer models seem unlikely for most of the remaining outer planets which suggests that these planets have a primordial hydrosphere. Our composition constraints also indicate that no planets are consistent with a core-free interior structure.

==> RESPONSE.tex <==
Again, we thank the referee very much for a thorough review and the useful comments that have improved the manuscript.  We have added more discussion to address the points raised.  New additions to the text are shown in red.

Reviewer's Comments:

Here is my review of ID:MN-22-5151-MJ.R1 "Composition constraints of the TRAPPIST-1 planets from their formation" by Childs et al.

First of all, I apologize for the delay in the report. The authors revised the manuscript according to my suggestions. This revision made it clear that this paper is weighted towards composition. Although their findings are more clear, I would like to ask for further clarification on the validity of the methods and the robustness of the conclusions.


>> #Major comments
>>
>> (b)Novelty of findings.
>>
>> Therefore, it is not clear what the new findings of this study are.
> 
> RESPONSE:  New findings from this paper include: 
> -the importance of fragmentation and the ability of fragments to seed entire planets through pebble accretion
> -a more specific formation history for the T1 planets (i.e the inner two planets grew most of their mass from collisions and the outer planets grew most of their mass by pebble accretion and the smaller planets may have been seeded by fragments)
> -inner planets experienced the most giant impacts and as a result, their volatile abundances should be lower, and their densities higher, than the outer planets
> -constraints on the refractory elements and their implications for the interior structure of the planets
> -Our composition constraints and interior model find two-layer solutions for planets b and c indicating that these planets do not have a volatile layer, but our results suggest the outer planets may need a volatile layer to match observed densities.
> -Additionally, our compositions constraints indicate now planets are consistent with a core-free interior.
> We have updated the conclusion and the abstract to better highlight these findings.

Their new findings are more clear. From this reply, as well as from the abstract and Section 7, it is clear that this paper is more focused on composition. Since some of these findings used the results of dust condensation calculations, I hope the authors discuss the validity of the method and the robustness of these findings, as described below.

RESPONSE:  We have added a discussion of the validity and robustness of using dust condensation results from the Solar System to Appendix B.

>> (c)Methodology.
>>
>> - About the disk model. The gas model uses Eqs.(1) and (4), and the pebble surface density uses Eq.(7). On the other hand, the initial compositions of planetesimals and pebbles use different surface density (Eq.21) and temperature (Eq.22). It is stated that the earlier phase is considered in the composition calculation, but there is no justification for using different disks. In addition, I wonder if the position of the snow line at 0.1 au agrees with Eq.(22).
> 
> RESPONSE:  The planetesimals will have a different surface density than the gas profile since they primarily form just exterior to the ice line.  The formation of these large solid bodies leads to decoupling from the gas disc to some degree.  We have added this to Section 3.  The locations of the ice line in the disc used in Eq. 22 will be further out than 0.1 au as this disc is meant to model disc evolution shortly after disc formation when the disc is much hotter.   We use different discs since our model has been tailored for M-dwarfs and the condensation code has been tailored for Sun-like stars.  We attempted to implement our disc model into the condensation code but to no avail.  Future work is needed to make the condensation code compatible with systems around low mass stars however doing so proved to be beyond the scope of this current project.  We clarify this in Section 2.4.

I understand that in the dust condensation calculation, the authors cannot set up the disk to match the TRAPPIST-1 system, and the conditions for the Sun and the Solar disk are used. However, when the disk is initially 0.21 M_sun, the disk is more massive than the mass of the TRAPPIST-1. This is indeed very tricky. Since they calculate the dust composition using a disk that has evolved to some extent (Fig.4), it may not depend much on the initial disk mass. However, the stellar evolution and the disk evolution should differ to some extent for M-type and G-type stars (eg, Siess+2000, Bayo+2012, Ansdell+2017, Picogna+2021). In addition, the authors adopted t~130kyr in Fig.4, but it is not clear why this is reasonable setting for the TRAPPIST-1 system (although there is an argument that it is consistent with chondrites in the solar system). 

RESPONSE:  We believe it is reasonable to rescale dust condensation results from the Solar System to an M-dwarf with a Solar-like composition, which is the case for T1 (see Delrez+ 2018).  While differences in the dust evolution will certainly arise from the differences in stellar evolution, we are interested only in the relative abundances at a single epoch which we use for our composition analysis.  Besides the initial composition in the disc, the relative abundances in the condensed dust should be only sensitive to local conditions when the temperature is above the condensation temperature.  When the temperature drops below condensation temperature, the relative abundances in the condensed dust become slowly varying function of local density and pressure.  We have added a discussion of this to Appendix B and show the rho, P, and T profiles between the re-scaled solar system disc and our disc here for comparison purposes.

As noted in point(b) above, the focus of this paper is on the composition, which is based on the results of this dust condensation calculation. Therefore, I hope that the authors could add a discussion of the validity of this setting and the robustness of how changing this setting would change the conclusions (eg, Table 3, Fig.5, Section 5.0.2).

RESPONSE:  We have added a discussion to Section 2.4 about the validity of assuming the relative abundances of the dust at a single epoch around a G-type star.  While we extrapolate the dust results at a single epoch and re-scale for disc size for technical reasons, we do expect the compositions of the bodies to change between G-type and M-dwarf systems if we were to more realistically model how these bodies chemically evolve in an evolving disc.  To understand the extent to which the compositions change between these two systems in this scenario requires future work as it is strongly coupled to disc evolution (specifically the mid-plane pressure and temperature profile).


>> - About the expression of the PIM. The reproduction of the mass distribution is one focus of this study. However, as stated in Section 5, the planetary mass is affected by the PIM. Therefore, the formula of the PIM is important. As mentioned in Schoonenberg+(2019), the PIM differs by several factors depending on the PIM model. I hope the authors explain why they chose Eq.(12) for the PIM. Also, in this case they consider a constant temperature distribution, but in reality the temperature should decrease with time. The authors would also comment on this.
>
> RESPONSE:  We use a more up-to-date expression for the PIM than previous studies.  We also included a discussion of the temperature dependence in the Discussion.  For future work, we will couple this code with a stellar evolution model and updated temperature profile so we may more accurately track temperature and mention this in Section 5.

I agree with the authors. It would be good to see how the results would change if more detailed temperature structures are considered in future studies. By the way, regarding “up-to-date expression of the PIM,” Bitsch+(2018) also derived the formula of the PIM. The PIMs of Bitsch+(2018) and Ataiee+(2018) are somewhat different. And since Bitsch+(2018) did 3D simulations, I don’t think we can say that Ataiee+(2018) is better than Bitsch+(2018). If the authors have a reason for using Ataiee+(2018)’s model, they might want to describe it.

RESPONSE: Yes, thank you for bringing this study to our attention.  Ataiee+ 2018 do a comparison of their results to Bitsch+ 2018 in their Appendix A and generally find good agreement although their PIM values differ by a factor of 1.5-2.  Exploring how the Bitsch+2018 PIM will affect our results is an area of interest for future study.  We have added a discussion of this to Section 6.

>> #Minor comments
>>
>> 13. Eq.(22). I think 0.21 M_sun is a typo for 0.21 M_star. Then why do the authors use Mdisc=0.21 M_star? This is a bit large. What is the value of r0? Is this consistent with Eq.(1)?
> 
> RESPONSE:  The initial disc mass for Eq. 22 is indeed 0.21 M_sun.  This corresponds to the disc mass around a Sun like star immediately after disc formation.  High accretion rates onto the star quickly deplete the disc mass and after one evolution timescale, the disc mass is less than 20\% its initial disc mass (see Cassen 1996 Figure 2).  We use solar values because the code is written for a solar type star and we had difficulties converting it to a profile more compatible with an M-dwarf.  We find the dust profiles from a solar like star and then normalize those to fit our T1 disc.  We have clarified this in Section 2.4.

I would suggest that the authors explain a bit little more about how they normalized the dust profile to match the TRAPPIST-1 disk. There are descriptions at the end of the 2nd and 3rd paragraphs of Section 2.4, but they are not clear. As mentioned above, I believe this setting affects the composition, so I hope the authors add explanations.

RESPONSE:  We have added details about how we re-scale the disc to Appendix B.


>> 16. The 2nd paragraph. Why is the orbital inclination extremely small compared to the orbital eccentricity?
>
> RESPONSE:  Both the eccentricity and the inclination are quite small as Moon-sized bodies will have damped orbits by interactions with the gas.  This point has been added to Section 3.

I ask why the eccentricity has a maximum of 5.7 degrees and the inclination has a maximum of 0.5 degrees. If the authors have a reason, they could state it. Coleman+(2019) has a maximum eccentricity of 0.57 degrees and a maximum inclination of 0.25 degrees, which are normal.

RESPONSE: Yes, our eccentricity is relatively high compared to Coleman+ 2019 and other similar studies however, our choices are motivated by the findings of Schoonenberg+ 2019 who modeled the formation of planetesimals that initially form in a narrow region just exterior to the ice line from the streaming instability.  In this formation channel, the planetesimals experience scattering due to the high number density of the bodies which leads to excited eccentricities exterior to the ice line (see Figure 4. of Schoonenberg+ 2019).  Similar results were also seen from direct simulations of planetesimal formation by Schäfer et al. (2017).  The initial conditions of Coleman+2019 are consistent with core accretion studies of the solar system for bodies distributed across the entirety of the disc range (see Chambers 2011), which may not necessarily be consistent with our formation channel where the bodies begin much closer together in a narrow belt just exterior to the ice line.  Still, our starting values for eccentricity and inclination are small but similar to Schoonenberg+ 2019, we observe scattering and orbital excitement of the bodies at the start of the simulation.  However, shortly after this period of excitement the orbits do get dampened and the eccentricity moves to smaller values than the initial value of 0.1.   We have added a plot that shows the inclination and eccentricity evolution of the bodies (Figure 3) and added a new subsection 4.3 with a discussion of these findings.

>> 25. The 3rd paragraph of Section 4.4. Please explain the justification for assuming a WMF of 20%.
>
> RESPONSE:  We experimented with different initial WMF's and found that a 0.2 WMF best reproduced the observed planet radii with our planet interior solver.  We have added this to the text.

I would suggest that the authors describe the extent to which they experimented with many different initial WMFs.

RESPONSE: We have added to Section 3 that we experimented with 15\%, 20\%, 25\%, and 50\% WMFs.

>> 31. Fig.6. I wonder what happens if this figure is drawn with the horizontal axis of the final orbital position of each planet. Are the inner planets subject to more ocean evaporating impacts?
> 
> RESPONSE:  We have added the recommended plot to the paper.  Indeed, the inner most planets are subject to more ocean evaporating impacts.

Thank you for adding this figure. This result is not surprising, but it may explain why there is less volatile material on the inner planets. This might be good to investigate in more detail in a future study.

RESPONSE: Yes, we agree that it helps explain why there is less volatile material on the inner planets and will keep this in mind for future studies.
